Unsupervised Domain Adaptation with Dynamic Clustering and Contrastive Refinement for Gait Recognition

Gait recognition is an emerging identification technology that distinguishes individuals at long distances by analyzing individual walking patterns. Traditional techniques rely heavily on large-scale labeled datasets, which incurs high costs and significant labeling challenges. Recently, researchers have explored unsupervised gait recognition with clustering-based unsupervised domain adaptation methods and achieved notable success. However, these methods directly use pseudo-label generated by clustering and neglect pseudolabel noise caused by domain differences, which affects the effect of the model training process. To mitigate these issues, we proposed a novel model called GaitDCCR, which aims to reduce the influence of noisy pseudo labels on clustering and model training. Our approach can be divided into two main stages: clustering and training stage. In the clustering stage, we propose Dynamic Cluster Parameters (DCP) and Dynamic Weight Centroids (DWC) to improve the efficiency of clustering and obtain reliable cluster centroids. In the training stage, we employ the classical teacher-student structure and propose Confidence-based Pseudo-label Refinement (CPR) and Contrastive Teacher Module (CTM) to encourage noisy samples to converge towards clusters containing their true identities. Extensive experiments on public gait datasets have demonstrated that our simple and effective method significantly enhances the performance of unsupervised gait recognition, laying the foundation for its application in the real-world. We will release the code at https://github.com/YanSun-github/GaitDCCR upon acceptance.

==> C-ACM.tex <==
% \usepackage{color}
% \usepackage[normalem]{ulem}
% \usepackage{tabularray}
\definecolor{Alto}{rgb}{0.831,0.831,0.831}
\begin{table}
\centering
\caption{Rank-1 (\%) comparison on CASIA-B. The best results of the model with different backbones and clothing conditions are highlighted in bold, and the second are marked with underline.}
\fontsize{9pt}{8pt}\selectfont
\label{C-ACM}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[120]Q[130]Q[200]Q[54]Q[54]Q[54]Q[54]Q[54]Q[54]Q[56]Q[56]Q[56]Q[56]Q[56]Q[63]},
  row{3} = {Alto,c},
  row{16} = {Alto,c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {r=2}{},
  cell{1}{4} = {c=11}{0.604\linewidth,c},
  cell{1}{15} = {r=2}{},
  cell{3}{1} = {c=15}{0.932\linewidth},
  cell{4}{1} = {r=4}{},
  cell{4}{2} = {r=4}{},
  cell{8}{1} = {r=4}{},
  cell{8}{2} = {r=4}{},
  cell{12}{2} = {r=4}{},
  cell{16}{1} = {c=15}{0.932\linewidth},
  cell{17}{1} = {r=12}{},
  cell{17}{2} = {r=4}{},
  cell{21}{2} = {r=4}{},
  cell{25}{2} = {r=4}{},
  cell{29}{1} = {r=12}{},
  cell{29}{2} = {r=4}{},
  cell{33}{2} = {r=4}{},
  cell{37}{2} = {r=4}{},
  hline{1,3-4,8,12,16-17,29,41} = {-}{},
  hline{2} = {4-14}{},
  hline{21,25,33,37} = {2-15}{},
}
Backbone                                                             & Condition & Method  & Probe View &      &      &      &      &      &      &      &      &      &      & Mean          \\
                                                                     &           &         & 0°         & 18°  & 36°  & 54°  & 72°  & 90°  & 108° & 126° & 134° & 162° & 180° &               \\
Fully supervised methods with all labels on CASIA-B                  &           &         &            &      &      &      &      &      &      &      &      &      &      &               \\
                                                                     & NM        & CNN-LB\cite{wu39comprehensive}  & 82.6       & 90.3 & 96.1 & 94.3 & 90.1 & 87.4 & 89.9 & 94.0 & 94.7 & 91.3 & 78.5 & 89.9          \\
                                                                     &           & GaitSet\cite{chao2021gaitset} & 90.8       & 97.9 & 99.4 & 96.9 & 93.6 & 91.7 & 95.0 & 97.8 & 98.9 & 96.8 & 85.8 & 95.0          \\
                                                                     &           & MT3D\cite{lin2020gait}    & 95.7       & 98.2 & 99.0 & 97.5 & 95.1 & 93.9 & 9.1  & 98.6 & 99.2 & 98.2 & 92.0 & \uline{96.7}  \\
                                                                     &           & GaitGL\cite{lin2022gaitgl}  & 96.0       & 98.3 & 99.0 & 97.9 & 96.9 & 95.4 & 97.0 & 98.9 & 99.3 & 98.8 & 94.0 & \textbf{97.4} \\
                                                                     & BG        & CNN-LB\cite{wu39comprehensive}  & 64.2       & 80.6 & 82.7 & 76.9 & 64.8 & 63.1 & 68.0 & 76.9 & 82.2 & 75.4 & 61.3 & 72.4          \\
                                                                     &           & GaitSet\cite{chao2021gaitset} & 83.8       & 91.2 & 91.8 & 88.8 & 83.3 & 81.0 & 84.1 & 90.0 & 92.2 & 94.4 & 79.0 & 87.2          \\
                                                                     &           & MT3D\cite{lin2020gait}    & 91.0       & 95.4 & 97.5 & 94.2 & 92.3 & 86.9 & 91.2 & 95.6 & 97.3 & 96.4 & 86.6 & \uline{93.0}  \\
                                                                     &           & GaitGL\cite{lin2022gaitgl}  & 92.6       & 96.6 & 96.8 & 95.5 & 93.5 & 89.3 & 92.2 & 96.5 & 98.2 & 96.9 & 91.5 & \textbf{94.5} \\
                                                                     & CL        & CNN-LB\cite{wu39comprehensive}  & 37.7       & 57.2 & 66.6 & 61.1 & 55.2 & 54.6 & 55.2 & 59.1 & 58.9 & 48.8 & 39.4 & 54.0          \\
                                                                     &           & GaitSet\cite{chao2021gaitset} & 61.4       & 75.4 & 80.7 & 77.3 & 72.1 & 70.1 & 71.5 & 73.5 & 73.5 & 68.4 & 50.0 & 70.4          \\
                                                                     &           & MT3D\cite{wu39comprehensive}    & 76.0       & 87.6 & 89.8 & 85.0 & 81.2 & 75.7 & 81.0 & 84.5 & 85.4 & 82.2 & 68.1 & \uline{81.5}  \\
                                                                     &           & GaitGL\cite{lin2022gaitgl}  & 76.6       & 90.0 & 90.3 & 87.1 & 84.5 & 79.0 & 84.1 & 87.0 & 87.3 & 84.4 & 69.5 & \textbf{83.6} \\
Unsupervised Domain Adaptation methods without any labels on CASIA-B &           &         &            &      &      &      &      &      &      &      &      &      &      &               \\
GaitSet                                                              & NM        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 87.1          \\
                                                                     &           & GaitSF\cite{ren2023unsupervised}  & 85.2       & 93.6 & 96.4 & 93.8 & 90.0 & 84.6 & 89.6 & 92.3 & 96.9 & 93.2 & 77.4 & 90.3          \\
                                                                     &           & STAGait\cite{ma2023fine} & 84.7       & 95.8 & 97.2 & 95.8 & 95.1 & 92.9 & 94.8 & 96.1 & 97.3 & 96.6 & 79.2 & \textbf{93.2} \\
                                                                     &           & Ours    & 76.7       & 93.8 & 95.4 & 94.1 & 89.5 & 85.2 & 87.6 & 91.1 & 93.1 & 89.5 & 78.1 & \uline{90.4}  \\
                                                                     & BG        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 68.1          \\
                                                                     &           & GaitSF\cite{ren2023unsupervised}  & 78.5       & 88.3 & 89.8 & 88.0 & 83.5 & 76.4 & 80.5 & 83.5 & 85.8 & 84.8 & 72.9 & \uline{82.9}  \\
                                                                     &           & STAGait\cite{ma2023fine} & 77.5       & 87.5 & 90.0 & 89.2 & 86.2 & 81.2 & 87.1 & 89.9 & 94.1 & 91.1 & 70.9 & \textbf{85.9} \\
                                                                     &           & Ours    & 73.5       & 80.2 & 83.3 & 80.8 & 75.8 & 69.4 & 72.5 & 81.1 & 79.3 & 79.6 & 62.3 & 80.1          \\
                                                                     & CL        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 27.2          \\
                                                                     &           & GaitSF\cite{ren2023unsupervised}  & 33.1       & 41.6 & 46.4 & 47.6 & 46.7 & 41.2 & 44.7 & 43.3 & 45.6 & 35.8 & 22.5 & \uline{40.8}  \\
                                                                     &           & STAGait\cite{ma2023fine} & 24.2       & 38.9 & 42.3 & 39.6 & 41.1 & 38.1 & 37.9 & 43.3 & 43.4 & 29.6 & 25.4 & 36.7          \\
                                                                     &           & Ours    & 21.8       & 38.4 & 45.5 & 43.1 & 42.1 & 37.7 & 36.7 & 33.1 & 35.5 & 26.1 & 20.2 & \textbf{42.8} \\
GaitGL                                                               & NM        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & \uline{92.8}  \\
                                                                     &           & GaitSF\cite{ren2023unsupervised}  & 84.2       & 95.7 & 96.2 & 94.7 & 89.9 & 87.1 & 89.1 & 91.8 & 96.7 & 93.2 & 63.6 & 89.3          \\
                                                                     &           & STAGait\cite{ma2023fine} & 76.7       & 88.3 & 88.8 & 87.1 & 88.4 & 82.9 & 85.9 & 90.6 & 93.1 & 93.9 & 73.0 & 86.2          \\
                                                                     &           & Ours    & 91.6       & 96.9 & 98.2 & 97.4 & 94.9 & 91.7 & 95.1 & 97.7 & 98.1 & 97.7 & 93.4 & \textbf{96.5} \\
                                                                     & BG        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 80.9          \\
                                                                     &           & GaitSF\cite{ren2023unsupervised}  & 75.8       & 90.1 & 91.6 & 87.5 & 83.9 & 80.2 & 83.0 & 85.0 & 89.7 & 87.9 & 56.1 & \uline{82}.8  \\
                                                                     &           & STAGait\cite{ma2023fine} & 69.1       & 85.3 & 84.7 & 83.6 & 82.9 & 76.1 & 79.9 & 86.8 & 89.1 & 88.1 & 63.6 & 80.8          \\
                                                                     &           & Ours    & 86.3       & 96.1 & 96.1 & 92.2 & 88.3 & 82.6 & 87.3 & 94.3 & 95.6 & 96.2 & 85.9 & \textbf{92.7} \\
                                                                     & CL        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 44.6          \\
                                                                     &           & GaitSF\cite{ren2023unsupervised}  & 53.6       & 71.1 & 76.9 & 75.5 & 72.9 & 69.1 & 69.8 & 69.1 & 71.7 & 60.7 & 31.2 & \uline{65.6}  \\
                                                                     &           & STAGait\cite{ma2023fine} & 43.9       & 65.3 & 66.5 & 66.9 & 68.8 & 60.0 & 66.4 & 71.2 & 69.3 & 61.8 & 42.2 & 62.0          \\
                                                                     &           & Ours    & 49.5       & 81.2 & 81.4 & 76.3 & 69.7 & 68.3 & 68.2 & 77.4 & 76.1 & 66.3 & 60.9 & \textbf{70.1} 
\end{tblr}
\end{table}

==> CASIA-B.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Rank-1 (\%) comparison on CASIA-B. The best results of the model with different backbones and clothing conditions are highlighted in bold, and the second are marked with underline.}
\fontsize{8pt}{6pt}\selectfont
\label{CAISA-B}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[110]Q[120]Q[200]Q[54]Q[54]Q[54]Q[54]Q[54]Q[54]Q[56]Q[56]Q[56]Q[56]Q[56]Q[63]},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {r=2}{},
  cell{1}{4} = {c=11}{0.604\linewidth,c},
  cell{1}{15} = {r=2}{},
  cell{3}{1} = {r=12}{},
  cell{3}{2} = {r=4}{},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{3}{10} = {c},
  cell{3}{11} = {c},
  cell{3}{12} = {c},
  cell{3}{13} = {c},
  cell{3}{14} = {c},
  cell{7}{2} = {r=4}{},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{7}{7} = {c},
  cell{7}{8} = {c},
  cell{7}{9} = {c},
  cell{7}{10} = {c},
  cell{7}{11} = {c},
  cell{7}{12} = {c},
  cell{7}{13} = {c},
  cell{7}{14} = {c},
  cell{11}{2} = {r=4}{},
  cell{15}{1} = {r=12}{},
  cell{15}{2} = {r=4}{},
  cell{15}{4} = {c},
  cell{15}{5} = {c},
  cell{15}{6} = {c},
  cell{15}{7} = {c},
  cell{15}{8} = {c},
  cell{15}{9} = {c},
  cell{15}{10} = {c},
  cell{15}{11} = {c},
  cell{15}{12} = {c},
  cell{15}{13} = {c},
  cell{15}{14} = {c},
  cell{19}{2} = {r=4}{},
  cell{19}{4} = {c},
  cell{19}{5} = {c},
  cell{19}{6} = {c},
  cell{19}{7} = {c},
  cell{19}{8} = {c},
  cell{19}{9} = {c},
  cell{19}{10} = {c},
  cell{19}{11} = {c},
  cell{19}{12} = {c},
  cell{19}{13} = {c},
  cell{19}{14} = {c},
  cell{23}{2} = {r=4}{},
  cell{23}{4} = {c},
  cell{23}{5} = {c},
  cell{23}{6} = {c},
  cell{23}{7} = {c},
  cell{23}{8} = {c},
  cell{23}{9} = {c},
  cell{23}{10} = {c},
  cell{23}{11} = {c},
  cell{23}{12} = {c},
  cell{23}{13} = {c},
  cell{23}{14} = {c},
  hline{1,3,27} = {-}{},
  hline{2} = {4-14}{},
  hline{7,11,15,19,23} = {2-15}{},
}
Backbone & Condition & Method  & Probe View &      &      &      &      &      &      &      &      &      &      & Mean          \\
         &           &         & 0°         & 18°  & 36°  & 54°  & 72°  & 90°  & 108° & 126° & 134° & 162° & 180° &               \\
GaitSet  & NM        & GOUDA\cite{habib2023watch}   & -          & -~   & -    & -    & -    & -    & -    & -    & -    & -    & -    & 87.1          \\
         &           & GaitSF\cite{ren2023unsupervised}  & 85.2       & 93.6 & 96.4 & 93.8 & 90.0 & 84.6 & 89.6 & 92.3 & 96.9 & 93.2 & 77.4 & 90.3          \\
         &           & STAGait\cite{ma2023fine} & 84.7       & 95.8 & 97.2 & 95.8 & 95.1 & 92.9 & 94.8 & 96.1 & 97.3 & 96.6 & 79.2 & \textbf{93.2} \\
         &           & Ours    & 76.7       & 93.8 & 95.4 & 94.1 & 89.5 & 85.2 & 87.6 & 91.1 & 93.1 & 89.5 & 78.1 & \uline{90.4}  \\
         & BG        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 68.1          \\
         &           & GaitSF\cite{ren2023unsupervised}  & 78.5       & 88.3 & 89.8 & 88.0 & 83.5 & 76.4 & 80.5 & 83.5 & 85.8 & 84.8 & 72.9 & \uline{82.9}  \\
         &           & STAGait\cite{ma2023fine} & 77.5       & 87.5 & 90.1 & 89.2 & 86.2 & 81.2 & 87.1 & 89.9 & 94.1 & 91.1 & 70.9 & \textbf{85.9} \\
         &           & Ours    & 73.5       & 80.2 & 83.3 & 80.8 & 75.8 & 69.4 & 72.5 & 81.1 & 79.3 & 79.6 & 62.3 & 80.1          \\
         & CL        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -~   & -    & -    & -    & 27.2          \\
         &           & GaitSF\cite{ren2023unsupervised}  & 33.1       & 41.6 & 46.4 & 47.6 & 46.7 & 41.2 & 44.7 & 43.3 & 45.6 & 35.8 & 22.5 & \uline{40.8}          \\
         &           & STAGait\cite{ma2023fine} & 24.2       & 38.9 & 42.3 & 39.6 & 41.1 & 38.1 & 37.9 & 43.3 & 43.4 & 29.6 & 25.4 & 36.7  \\
         &           & Ours    & 21.8       & 38.4 & 45.5 & 43.1 & 42.1 & 37.7 & 36.7 & 33.1 & 35.5 & 26.1 & 20.2 & \textbf{42.8} \\
GaitGL   & NM        & GOUDA\cite{wang2023dygait}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & \uline{92.8}  \\
         &           & GaitSF\cite{ren2023unsupervised}  & 84.2       & 95.7 & 96.2 & 94.7 & 89.9 & 87.1 & 89.1 & 91.8 & 96.7 & 93.2 & 63.6 & 89.3          \\
         &           & STAGait\cite{ma2023fine} & 76.7       & 88.3 & 88.8 & 87.1 & 88.4 & 82.9 & 85.9 & 90.6 & 93.1 & 93.9 & 73.0 & 86.2          \\
         &           & Ours    & 91.6       & 96.9 & 98.2 & 97.4 & 94.9 & 91.7 & 95.1 & 97.7 & 98.1 & 97.7 & 93.4 & \textbf{96.5} \\
         & BG        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 80.9          \\
         &           & GaitSF\cite{ren2023unsupervised}  & 75.8       & 90.1 & 91.6 & 87.5 & 83.9 & 80.2 & 83.0 & 85.0 & 89.7 & 87.9 & 56.1 & \uline{82.8}  \\
         &           & STAGait\cite{ma2023fine} & 69.1       & 85.3 & 84.7 & 83.6 & 82.9 & 76.1 & 79.9 & 86.8 & 89.1 & 88.1 & 63.6 & 80.8          \\
         &           & Ours    & 86.3       & 96.1 & 96.1 & 92.2 & 88.3 & 82.6 & 87.3 & 94.3 & 95.6 & 96.2 & 85.9 & \textbf{92.7} \\
         & CL        & GOUDA\cite{habib2023watch}   & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & 44.6          \\
         &           & GaitSF\cite{ren2023unsupervised}  & 53.6       & 71.1 & 76.9 & 75.5 & 72.9 & 69.1 & 69.8 & 69.1 & 71.7 & 60.7 & 31.2 & \uline{65.6}  \\
         &           & STAGait\cite{ma2023fine} & 43.9       & 65.3 & 66.5 & 66.9 & 68.8 & 60.0 & 66.4 & 71.2 & 69.3 & 61.8 & 42.2 & 62.0            \\
         &           & Ours    & 49.5       & 81.2 & 81.4 & 76.3 & 69.7 & 68.3 & 68.2 & 77.4 & 76.1 & 66.3 & 60.9 & \textbf{70.1} 
\end{tblr}
\end{table}

==> OUMVLP.tex <==
% \usepackage[normalem]{ulem}
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Rank-1 (\%) comparison on OUMVLP in various view angles. The best results are highlighted in bold, and the second are marked with underline.}
% \fontsize{8pt}{10pt}\selectfont
\label{OUMVLP}
\begin{tblr}{
  width = \linewidth,
  colspec = {Q[180]Q[140]Q[200]Q[40]Q[40]Q[40]Q[40]Q[40]Q[40]Q[40]Q[45]Q[45]Q[45]Q[45]Q[45]Q[45]Q[45]Q[20]},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {r=2}{},
  cell{1}{4} = {c=14}{0.658\linewidth,c},
  cell{1}{18} = {r=2}{},
  cell{3}{1} = {r=4}{},
  cell{3}{2} = {r=2}{},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{3}{10} = {c},
  cell{3}{11} = {c},
  cell{3}{12} = {c},
  cell{3}{13} = {c},
  cell{3}{14} = {c},
  cell{3}{15} = {c},
  cell{3}{16} = {c},
  cell{3}{17} = {c},
  cell{5}{2} = {r=2}{},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{5}{10} = {c},
  cell{5}{11} = {c},
  cell{5}{12} = {c},
  cell{5}{13} = {c},
  cell{5}{14} = {c},
  cell{5}{15} = {c},
  cell{5}{16} = {c},
  cell{5}{17} = {c},
  cell{7}{1} = {r=4}{},
  cell{7}{2} = {r=2}{},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{7}{7} = {c},
  cell{7}{8} = {c},
  cell{7}{9} = {c},
  cell{7}{10} = {c},
  cell{7}{11} = {c},
  cell{7}{12} = {c},
  cell{7}{13} = {c},
  cell{7}{14} = {c},
  cell{7}{15} = {c},
  cell{7}{16} = {c},
  cell{7}{17} = {c},
  cell{9}{2} = {r=2}{},
  cell{9}{4} = {c},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{9}{7} = {c},
  cell{9}{8} = {c},
  cell{9}{9} = {c},
  cell{9}{10} = {c},
  cell{9}{11} = {c},
  cell{9}{12} = {c},
  cell{9}{13} = {c},
  cell{9}{14} = {c},
  cell{9}{15} = {c},
  cell{9}{16} = {c},
  cell{9}{17} = {c},
  hline{1,3,7,11} = {-}{},
  hline{2} = {4-17}{},
  hline{5,9} = {2-18}{},
}
Source Dataset & Backbone & Method & Probe View &      &      &      &      &      &      &      &      &      &      &      &      &      & Mean          \\
               &          &        & 0°         & 15°  & 30°  & 45°  & 60°  & 75°  & 90°  & 180° & 195° & 210° & 225° & 240° & 255° & 270° &               \\
CASIA-B        & GaitSet  & GOUDA\cite{habib2023watch}  & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & \uline{27.9}  \\
               &          & Ours   & 24.6       & 44.1 & 50.9 & 51.1 & 45.5 & 46.1 & 43.2 & 28.2 & 44.4 & 49.8 & 50.8 & 44.6 & 44.7 & 39.3 & \textbf{43.6} \\
               & GaitGL   & GOUDA\cite{habib2023watch}  & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & \uline{34.1}  \\
               &          & Ours   & 28.9       & 48.3 & 55.4 & 55.9 & 51.4 & 52.3 & 48.8 & 30.5 & 44.9 & 53.1 & 53.1 & 48.9 & 47.6 & 43.8 & \textbf{49.2} \\
GREW           & GaitSet  & GOUDA\cite{habib2023watch}  & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & \uline{38.8}  \\
               &          & Ours   & 47.9       & 68.3 & 76.2 & 78.5 & 69.5 & 68.2 & 64.2 & 51.6 & 68.7 & 75.7 & 78.8 & 73.4 & 71.7 & 66.3 & \textbf{68.5} \\
               & GaitGL   & GOUDA\cite{habib2023watch}  & -          & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & -    & \uline{44.2}  \\
               &          & Ours   & 40.5       & 58.0 & 65.4 & 67.3 & 63.1 & 64.1 & 60.8 & 44.1 & 58.4 & 67.4 & 67.9 & 65.8 & 63.9 & 61.7 & \textbf{60.6} 
\end{tblr}
\end{table}
